Deep Gaussian Denoiser Epistemic Uncertainty and Decoupled Dual-Attention Fusion

Following the performance breakthrough of denoising networks, improvements have come chiefly through novel architecture designs and increased depth. While novel denoising networks were designed for real images coming from different distributions, or for specific applications, comparatively small improvement was achieved on Gaussian denoising. The denoising solutions suffer from epistemic uncertainty that can limit further advancements. This uncertainty is traditionally mitigated through different ensemble approaches. However, such ensembles are prohibitively costly with deep networks, which are already large in size. Our work focuses on pushing the performance limits of state-of-the-art methods on Gaussian denoising. We propose a model-agnostic approach for reducing epistemic uncertainty while using only a single pretrained network. We achieve this by tapping into the epistemic uncertainty through augmented and frequency-manipulated images to obtain denoised images with varying error. We propose an ensemble method with two decoupled attention paths, over the pixel domain and over that of our different manipulations, to learn the final fusion. Our results significantly improve over the state-of-the-art baselines and across varying noise levels.

==> clipping_ablation_table.tex <==
\begin{table*}[t]
	\centering
	\scriptsize
	\begin{tabular}{c|c|c|c|c|c|c|c}
		\toprule
		Denoiser & \makecell[c]{Noise\\Level} 
		& \makecell[c]{Baseline\\w/ clip}
		& \makecell[c]{Simple average\\w/ clip} 
		& \makecell[c]{Our method\\w/ clip} 
		& \makecell[c]{Baseline\\w/o  clip}
		& \makecell[c]{Simple average\\w/o clip} 
		& \makecell[c]{Our method\\w/o clip} 
		\\
		\cline{1-8}
		
		\parbox[t]{5mm}{\multirow{5}{*}{\rotatebox[origin=l]{90}{\makecell[c]{DnCNN~\cite{zhang2017beyond}\\train w/o clip}}}}  
		& 10 & 33.30 & 33.11 & 33.60 & 33.33 & 33.14 &33.63\\
		& 20 & 29.72 & 29.67 & 30.02 & 29.89 & 29.82 &30.06\\
		& 30 & 27.68 & 27.66 & 28.15 & 28.09 & 28.02 &28.21\\
		& 40 & 26.19 & 26.18 & 26.91 & 26.88 & 26.79 &26.98 \\
		& 50 & 24.96 & 24.96 & 25.99 & 25.97 & 25.86 &26.09\\
        \cline{1-8}
        
		\parbox[t]{5mm}{\multirow{5}{*}{\rotatebox[origin=l]{90}{\makecell[c]{DnCNN~\cite{zhang2017beyond}\\train w/ clip}}}} 
		& 10 & 33.28 & 33.15 & 33.52 & 31.56 & 31.80 & 33.26\\
		& 20 & 29.55 & 29.58 & 29.91 & 23.66 & 24.73 & 29.59\\
		& 30 & 27.35 & 27.47 & 28.14 & 17.10 & 18.71 & 27.66\\
		& 40 & 25.67 & 25.90 & 26.91 & 12.10 & 13.73 & 26.19\\
		& 50 & 24.24 & 24.60 & 26.01 & 8.85  & 10.29 & 24.91\\
		\bottomrule
	\end{tabular}
	\caption{Effects of clipping}
	\label{table:effect_clip}
\end{table*}



==> color_DnCNN_table.tex <==
\centering
\begin{table*}[t]
	\centering
	\setulcolor{red}
	\setul{0.25ex}{0.25ex}
	\begin{tabular}{ccccc}
		\toprule
		\makecell[c]{Backbone\\denoiser}
		& \makecell[c]{Noise\\level} 
		& \makecell[c]{Baseline\\result} 
		& \makecell[c]{Ensemble\\(SM - FM - Joint)}
		& \makecell[c]{Ours full\\(SM - FM - Joint)} \\ \cline{1-5}
		\noalign{\smallskip}
		
		\multirow{5}{*}{CDnCNN~\cite{zhang2017beyond}}
		& 10 & 35.35 & 35.50 33.92 35.14 & 35.61 35.49 \textbf{35.68} \\
		& 20 & 31.27 & 31.38 30.91 31.35 & 31.79 31.83 \textbf{31.85} \\
		& 30 & 28.76 & 28.84 28.85 28.98 & 29.81 29.64 \textbf{29.87} \\
		& 40 & 26.80 & 26.87 27.23 27.15 & 28.49 28.50 \textbf{28.53} \\
		& 50 & 25.09 & 25.15 25.82 25.57 & 27.50 27.47 \textbf{27.56} \\
		\noalign{\smallskip}
		
		\bottomrule 
	\end{tabular}
	\caption{Color Gaussian denoising PSNR ($dB$) results with the CDnCNN backbone, the averaging ensemble, and our full dual model. We include the ablations using only our spatially-manipulated (SM) or frequency-manipulated (FM) images, rather than all (Joint). The best results are highlighted in bold.}
	\label{table:colorden_psnr_results}
\end{table*}
